Nimble: Efficiently Compiling Dynamic Neural Networks for Model Inference

Modern deep neural networks increasingly make use of features such as dynamic control flow, data structures and dynamic tensor shapes. Existing deep learning systems focus on optimizing and executing static neural networks which assume a pre-determined model architecture and input data shapes--assumptions which are violated by dynamic neural networks. Therefore, executing dynamic models with deep learning systems is currently both inflexible and sub-optimal, if not impossible. Optimizing dynamic neural networks is more challenging than static neural networks; optimizations must consider all possible execution paths and tensor shapes. This paper proposes Nimble, a high-performance and flexible system to optimize, compile, and execute dynamic neural networks on multiple platforms. Nimble handles model dynamism by introducing a dynamic type system, a set of dynamism-oriented optimizations, and a light-weight virtual machine runtime. Our evaluation demonstrates that Nimble outperforms state-of-the-art deep learning frameworks and runtime systems for dynamic neural networks by up to 20x on hardware platforms including Intel CPUs, ARM CPUs, and Nvidia GPUs.

==> figs/memory.tex <==
\pgfplotstableread{./data/memory.dat}\memory
\begin{tikzpicture}
    \tikzset{
        hatch distance/.store in=\hatchdistance,
        hatch distance=10pt,
        hatch thickness/.store in=\hatchthickness,
        hatch thickness=2pt,
        %hatch shift/.store in=\hatchshift,
        %hatch shift=1pt,
        %hatch spread/.store in=\hatchspread,
        %hatch spread=3pt
    }
    \makeatletter
    \definecolor{barfillgray}{gray}{0.75}  
    \begin{axis}[
       	ybar=0pt, %no gap between bars
        height=0.3\textwidth,
        width=0.5\textwidth,
%        scale=0.65,
        bar width=10pt,
        %xlabel=Benchmarks,
        %ymajorgrids = true,
        major x tick style = transparent,
        xtick=data,
        enlarge x limits=0.2,
		ymin=0,
		ymax=2.5,
		ytick={0, 0.5, 1.0, 1.5, 2.0, 2.5},
		% Set the grid line
		extra y ticks=1,
        extra y tick style={grid=major, grid style={dashed,black}},
        ylabel = Relative memory usage,
        %ylabel style = {yshift=-8pt},
        ylabel near ticks,
        %xlabel style = {yshift=-4ex},
        xticklabels={ResNet, MobileNet, VGG, SqueezeNet},
		every axis/.append style={font=\small},
		legend style={at={(0.905, 1.21)},font=\small},
		%legend style={at={(0.555, 1.2)},font=\small}, %for height=0.2\textwidth,
        legend columns=3,
        legend cell align = left,
		legend image code/.code={%
      		\draw[#1] (0cm,-0.1cm) rectangle (0.2cm,0.08cm);
    	},
	]
     	\addplot [draw=black, pattern=flexible hatch, hatch distance=8pt, hatch thickness=1.2pt] table[x expr=\coordindex, y=NimbleNoMem] {\memory};
     	\addlegendentry{Nimble-no-memory}
     	\addplot [draw=black, pattern color=black, pattern=dots, hatch distance=10pt] table[x expr=\coordindex, y=NimbleMem] {\memory};
     	\addlegendentry{Nimble-memory}
     	\addplot [fill=barfillgray, hatch distance=5pt, hatch thickness=1pt] table[x expr=\coordindex, y=TVM] {\memory};
     	\addlegendentry{TVM}
    \end{axis}
\end{tikzpicture}

==> figs/memory_bak.tex <==
\subsection{Memory planning}
\label{sec:compliation:memory}

Many existing IRs do not make memory allocation explicit in their IRs, instead leaving it implicit and allocating memory at each node in combination with runtime system optimizations in order to efficiently use memory. 
Even when IRs do introduce explicit notions of memory, analyses only work well for graphs with static shape information, and no control-flow. Furthermore these passes are often rigid and non-compositional disallowing customization for new platforms or chaining with model-specific optimizations. A few approaches to DL memory optimizations use low-level concepts of memory to optimize, but it is important that memory optimizations occur at a suitably high-level of abstraction before essential program facts are lost. Furthermore as discussed in Section~\ref{sec:compilation:shape-func} we have introduced new ways to account for the handling of dynamic allocations which further complicate memory analysis.

In order to handle memory allocation for dynamic shapes we have introduced a set of memory extensions to the TVM front-end IR. Using these extension we can transform the extension into the standard functional dialect where operators return their results, and allocation is implicit to a dialect where all memory allocation is explicit. We change each operator invocation's calling convention to explicitly mark the input and output tensors, as well as making all allocation explicit.

In particular we introduced four new IR constructs, \verb|invoke_tvm_op(op, inputs, outputs)| which makes the TVM calling convention explicit, \texttt{allocate\_storage(size, alignment, attrs)} which allocates a region of memory with a particular size, \texttt{allocate\_tensor(storage, shape, dtype, attrs)} which allocates tensor from a given piece of storage with some shape and data type, and finally \verb|kill(tensor)| which frees a tensor before its reference count becomes zero due to exiting the frame. 

\begin{comment}
We can demonstrate how to transform a single statically shaped operation such as broadcasting addition.

\begin{Verbatim}[fontsize=\small]
fn @main() -> Tensor[(k,), f32] {
    let t1: Tensor[(10,), f32] = ...;
    let t2: Tensor[(10,), f32] = ...;
    // Implicitly allocates the output buffer of add
    add(t1, t2)
}
\end{Verbatim}

Here we only must allocate a single buffer, the return buffer for the addition operation.

\begin{Verbatim}[fontsize=\small]
fn @main() -> Tensor[(k,), f32] {
    let t1 = ...;
    let t2 = ...;
    let storage = alloc_storage(40, 64, f32);
    let out1 = alloc_tensor(storage, (10,), f32);
    invoke_tvm_op(add, (t1, t2), (out1,));
    out1
}
\end{Verbatim}
\end{comment}

After the initial transform we manifest a perfectly sized storage and allocate a tensor
directly from the storage at offset zero. The insight of this transformation is internalizing
memory allocation directly into the IR. Not only does this elegantly solve the static case,
subsuming existing memory planning passes, but can be generalized into a transform that
works in the presence of control and dynamic shapes.

The most challenging step of this transformation is handling dynamic shapes. Our handling of dynamic shape requires us to first compute the shape function from potentially fused kernels. As detailed in Section~\ref{sec:compilation:shape-func} our shape functions may require the input, the input \textit{shape}, or both. We would like to internalize the shape functions into the IR so that we may fuse both the allocation and computation into a single large kernel, eliminating the need for host synchronization when allocating. A side effect of our uniform treatment of shape functions as operators
is that we must also recursively manifest the allocations required to invoke the shape function. We illustrate this below, for example consider the program with a single dynamic concatenation.

\begin{Verbatim}[fontsize=\small]
fn (%x: Tensor[(?, 2), float32], 
    %y: Tensor[(1, 2), float32]) 
    -> Tensor[(?, 2), float32] 
{
  concatenate((%x, %y)) 
}
\end{Verbatim}

We have performed the same transformation as above, with the addition of carefully inserting 
invocations of the the shape function in order to manifest the output buffers required by invoking the
dynamically sized kernel. The below example is the code produced by the compiler today, with 
some storage size math and minor details omitted for clarity.

\begin{Verbatim}[fontsize=\small]
fn (%x: Tensor[(?, 2), float32], 
    %y: Tensor[(1, 2), float32]) 
    -> Tensor[(?, 2), float32] 
{
// The example below.
let %in_shape_0 = shape_of(%x, dtype="int64");
let %in_shape_1 = shape_of(%y, dtype="int64");
let %storage_0 = memory.alloc_storage(16, 64, ...);
let %shape_func_out_0 = 
  memory.alloc_tensor(
    %storage_0, 
    meta[relay.Constant][0], 
    ...);
%1 = fn (%p0, %p1) {
  concatenate(%p0, %p1)
};
let %shape_func = memory.shape_func(
    %1, 
    (%in_shape_0, %in_shape_1), 
    (%shape_func_out_0,), ...);
let %storage_01 = memory.alloc_storage(..., 64, ...);
let %out_0 = memory.alloc_tensor(
    %storage_01, %shape_func_out_0, ...);
let %v = memory.invoke_tvm_op(%1, (%x, %y), (%out_0,));
%out_0
}
\end{Verbatim}

After the initial transformation you may notice we have introduced the specialized \verb|memory.shape_func| which invokes a shape function for a provided fused kernel.
The shape function requires input shapes as its arguments which further require us to invoke \verb|shape_of| for both \verb|%x| and \verb|%y|. Our goal is to complete eliminate implicit 
allocations so we must transform the program in order to handle these calls. For the first line
of the function above is expanded as so:

\begin{Verbatim}[fontsize=\small]
let %storage_0 = memory.alloc_storage(16, 64, ...);
let %tensor_0 = memory.alloc_tensor(
  %storage_0, 
  meta[relay.Constant][0], ...);
%0 = fn (%p0) {
  shape_of(%p0, dtype="int64")
};
%1 = (%x,);
%2 = (%tensor_0,);
let %v = memory.invoke_tvm_op(%0, %1, %2);
\end{Verbatim}

After performing this transformation we can explicitly see all storage requirements, and analyze the liveness of all tensors including those used in both normal computation and shape functions. By manifesting these into the IR we enable further optimization downstream by both ourselves and future users. For example liveness analysis can be used to reuse storage, storage can be reclaimed and coalesced and so on.





==> figs/static_perf.tex <==
\pgfplotstableread{./data/staticperformance.dat}\staticperf
\begin{tikzpicture}
    \tikzset{
        hatch distance/.store in=\hatchdistance,
        hatch distance=10pt,
        hatch thickness/.store in=\hatchthickness,
        hatch thickness=2pt,
        %hatch shift/.store in=\hatchshift,
        %hatch shift=1pt,
        %hatch spread/.store in=\hatchspread,
        %hatch spread=3pt
    }
    \makeatletter
    \pgfdeclarepatternformonly[\hatchdistance,\hatchthickness]{flexible hatch}
    {\pgfqpoint{0pt}{0pt}}
    {\pgfqpoint{\hatchdistance}{\hatchdistance}}
    {\pgfpoint{\hatchdistance-1pt}{\hatchdistance-1pt}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\hatchthickness}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{\hatchdistance}{\hatchdistance}}
        \pgfusepath{stroke}
    }
    
    \pgfdeclarepatternformonly[\hatchdistance,\hatchthickness]{east hatch}
    {\pgfqpoint{-0pt}{-0pt}}
    {\pgfqpoint{3pt}{3pt}}
    {\pgfqpoint{3pt}{3pt}}
    {
        \pgfsetlinewidth{0.8pt}
        \pgfpathmoveto{\pgfqpoint{0pt}{3pt}}
        \pgfpathlineto{\pgfqpoint{3pt}{0pt}}
        \pgfpathmoveto{\pgfqpoint{.2pt}{-.2pt}}
        \pgfpathlineto{\pgfqpoint{-.2pt}{.2pt}}
        \pgfpathmoveto{\pgfqpoint{3.2pt}{2.8pt}}
        \pgfpathlineto{\pgfqpoint{2.8pt}{3.2pt}}
        \pgfusepath{stroke}
    }
    
    \definecolor{barfillgray}{gray}{0.75}  
    \begin{axis}[
       	ybar=0pt, %no gap between bars
        height=0.3\textwidth,
        width=0.5\textwidth,
%        scale=0.65,
        bar width=10pt,
        %xlabel=Benchmarks,
        %ymajorgrids = true,
        major x tick style = transparent,
        xtick=data,
        enlarge x limits=0.2,
		ymin=0,
		ymax=1.2,
		ytick={0, 0.5, 1.0},
		% Set the grid line
		extra y ticks=1,
        extra y tick style={grid=major, grid style={dashed,black}},
        ylabel = Relative latency,
        %ylabel style = {yshift=-8pt},
        ylabel near ticks,
        %xlabel style = {yshift=-4ex},
        xticklabels={ResNet, MobileNet, VGG, SqueezeNet},
		every axis/.append style={font=\small},
		legend style={at={(0.657, 1.21)},font=\small},
		%legend style={at={(0.555, 1.2)},font=\small}, %for height=0.2\textwidth,
        legend columns=4,
        legend cell align = left,
		legend image code/.code={%
      		\draw[#1] (0cm,-0.1cm) rectangle (0.2cm,0.08cm);
    	},
	]
     	\addplot [draw=black, pattern=flexible hatch, hatch distance=8pt, hatch thickness=1.2pt] table[x expr=\coordindex, y=Intel] {\staticperf};
     	\addlegendentry{Intel}
     	\addplot [draw=black, pattern color=black, pattern=dots, hatch distance=10pt] table[x expr=\coordindex, y=Nvidia] {\staticperf};
     	\addlegendentry{Nvidia}
     	\addplot [fill=barfillgray] table[x expr=\coordindex, y=ARM] {\staticperf};
     	\addlegendentry{ARM}
     	\addplot [draw=black, pattern color=black, pattern=east hatch, hatch distance=15pt] table[x expr=\coordindex, y=Baseline] {\staticperf};
     	\addlegendentry{Baseline}
    \end{axis}
\end{tikzpicture}


==> figs/table_isa.tex <==

\begin{comment}

\begin{tabular}{@{}ll@{}}
\toprule
Instruction                                                   & Description                                                                \\ \midrule
Move                                                          & Moves data from one register to another.                                    \\
Ret                                                           & Returns the object in register result to caller's register.                 \\
Invoke                                                        & Invokes a function at in index.                                               \\
InvokeClosure                                                 & Invokes a Relay closure.                                                      \\
InvokePacked                                                  & Invokes the function containing registered operators in TOPI.                \\
AllocStorage                                                  & Allocates a storage block.                                                  \\
AllocTensor                                                   & Allocates a tensor value of a certain shape.                                 \\
AllocTensorReg                                                & Allocates a tensor based on a register.                                      \\
AllocDatatype                                                 & Allocates a data type using the entries from a register.                     \\
AllocClosure                                                  & Allocates a closure with a lowered virtual machine function.                  \\
GetField                                                      & Gets the value at a certain index from an VM object.                          \\
GetTag                                                        & Gets the tag of an Algebraic Data Types (ADT) constructor.                    \\
If                                                            & Jumps to the true or false offset depending on the condition.                 \\
Goto                                                          & Unconditionally jumps to an offset.                                            \\
LoadConst                                                     & Loads a constant at an index from the constant pool.                         \\
LoadConsti                                                    & Loads a constant immediate.                                                  \\
DeviceCopy                                                    & Copy a chunk of data from one device to another.                             \\
ShapeOf                                                       & Compute the shape of a tensor.                                               \\
Fatal                                                         & Raises fatal in the VM.                                                      \\
\bottomrule
\end{tabular}


\end{comment}

\begin{tabular}{@{}p{0.1\textwidth}p{0.375\textwidth}p{0.1\textwidth}p{0.375\textwidth}@{}}
\toprule
Instruction    & Description                                                  & Instruction   & Description.                                            \\ \midrule
Move           & Moves data from one register to another.                     & GetField      & Gets the value at a certain index from an VM object.          \\
Ret            & the object in register result to caller's register.          & ReshapeTensor & Changes the shape of a tensor without altering its data.      \\
Invoke         & Invokes a function at an index.                              & If            & Jumps to the true or false offset with a condition.           \\
InvokeClosure  & Invokes a Relay closure.                                     & Goto          & Unconditionally jumps to an offset.                           \\
InvokePacked   & Invokes the function including operator kernel.              & LoadConst     & Loads a constant at an index from the constant pool.          \\
AllocStorage   & Allocates a storage block.                                   & LoadConsti    & Loads a constant immediate.                                   \\
AllocTensor    & Allocates a tensor value of a certain shape.                 & DeviceCopy    & Copies a chunk of data from one device to another.              \\
AllocTensorReg & Allocates a tensor based on a register.                      & ShapeOf       & Retrieves the shape of a tensor.                               \\
AllocADT.      & Allocates a data type using the entries from a register.     & Fatal         & Raises fatal in the VM.                                       \\
AllocClosure   & Allocates a closure. & GetTag        & Gets the tag of an Algebraic Data Types (\texttt{ADT}) cstr.       \\
\bottomrule
\end{tabular}


==> mlsys/overview.tex <==
\section{System Overview}
%\label{sec:overview}

\subsection{VM Design}
\zhicomment{Should have a better header here.}

In \system, the compiler mainly targets the tensor operations and the runtime dispatches the instructions to handle those tensor-level operations which internally may contain a large body of low-level machine instructions. We, hence, naturally select the register-based virtual machine design~\yida{need ref} so that the bytecode is compact. We also provide an abstraction to let the VM operate on infinite set of virtual registers. It significantly alleviates optimizations and memory allocation, etc.
 
% we probably want to talk about this in the instruction set or memory planning. No need to have a separate paragraph here.
%The design of \system focuses on the simplicity without sacrificing performance. In order to accomplish this, we design a tensor VM rather than a scalar VM. In the tensor VM setting, we optimize for cheap ``allocation'' of objects (by trying to avoid real allocation), reuse of static fragments, and the ability to support dynamic shape (i.e jagged tensors). \autoref{fig:vm} depicts the overview design of VM. It essentially contains a compiler and a runtime system. The compiler compiles a Relay program into both hardware dependent and hardware independent modules/libraries. The hardware independent code consists of low-level bytecode that is specifically designed for efficient execution of VM. The hardware dependent code is composed of coarse-grain operators registered in the TVM operator inventory (TOPI). The runtime system takes charge of the execution of generated bytecode, i.e. dispatching the instructions and managing the stack frame and registers. We will detail the design of the VM in the following sections.

%\zhicomment{@haichen,  Do you still need push and pop? I think we probably don't need them now, instead we use \textit{Move} to manage stack. Am I right?}
%\textit{stack-based} and \textit{register-based} virtual machines are the two major types of VM in programming languages. Stack-based VM aims at simplicity, using \textit{push} and \textit{pop} instructions to maintain a unified stack. However, it complicates tasks such as dataflow analysis and enforces certain orders in the execution. Instead, register-based VM design manages registers to designate the operands and results rather than the stack. This type of VM simplifies the calling convention as values are carried by registers. But it may bring some cost in terms of code size as it needs to decode instructions to fetch the values at specific positions. As aforementioned that our VM mainly targets tensor-level instructions instead of low-level machine instructions. The code size is thus generally small. Furthermore, we would emphasize the convenience of optimizations, such as liveness analysis and memory allocation in the model inference scenario. Therefore, the register-based VM provides more benefits which meets our selection.

%\subsubsection{Instruction Set}

Instruction set is another important design for VM. \autoref{tab:isa} summarizes the instruction set we propose in the virtual machine. The choices of an instruction set and instruction representation are one of the most critical design decisions for a VM. The current representation of the instructions is a tagged union containing the op-code and the data payload. An important design decision is the architectural complexity (RISC vs. CISC) and the instruction encoding format (fixed-length encoding vs. variable-length encoding). \system's instruction set is closer to CISC to allow one single instruction to execute multiple ``low-level'' operations. For example, \texttt{LoadConst idx, \$reg} is essentially capable of multiple addressing modes as it first reads the index \texttt{idx} and then loads the data from a constant pool to the destination register \texttt{\$reg}. \system also adopted the variable-length instruction format due to the inclusion of the shape as the part of the instruction. 

\begin{table*}[t]
\centering
\input{figs/table_isa}
\caption{The opcode and the description of the \system instruction set \label{tab:isa}}
\end{table*}

This design has the following benefits. First, both CISC-style instruction and variable length encoding can lead to better code density. This advantage is of significance for edge devices that only have limited resources. Second, allowing multiple addressing modes to execute a single instruction may reduce the amount of data fetched from cache hierarchy and main memory. It could also possibly lead to better spatial locality as the data (e.g. the tensor value) may remain in the cache. Third, variable-length instruction encoding paves the avenue for extending extra information to instructions, e.g. debugging and even branch prediction. Last but not least, the low level instruction design in \system effectively separates hardware-dependent kernels from model control logic. That being said, the bytecode of \system is hardware-independent, although the kernels being invoked by the \texttt{InvokePacked} instruction is hardware-dependent. It eases the task of bytecode serialization.

% Instruction and bytecode design.

%\subsection{Kernel dispatch}

%\subsection{Memory management}
